Statistical Analysis of Inter Coding in VVC Test Model (VTM)

The promising improvement in compression efficiency of Versatile Video Coding (VVC) compared to High Efficiency Video Coding (HEVC) comes at the cost of a non-negligible encoder side complexity. The largely increased complexity overhead is a possible obstacle towards its industrial implementation. Many papers have proposed acceleration methods for VVC. Still, a better understanding of VVC complexity, especially related to new partitions and coding tools, is desirable to help the design of new and better acceleration methods. For this purpose, statistical analyses have been conducted, with a focus on Coding Unit (CU) sizes and inter coding modes.

==> result.tex <==
\begin{table*}[t]
\centering
\caption{\label{tab:Result}Performance of the proposed method in comparison with reference CNN-based methods (Unit: \%)}        
\begin{tabular}{c|c|cc|cc|cc|cc}
\hline 
\hline
\multirow{2}{*}{Class} &    \multirow{2}{*}{Sequence}      & \multicolumn{2}{c|}{Pan \cite{pan2021cnn} \scriptsize{(VTM6)}} & \multicolumn{2}{c|}{Yeo \cite{yeo2021cnn} \scriptsize{(VTM11)}} & \multicolumn{2}{c|}{Proposed (Th=0)} & \multicolumn{2}{c}{Proposed (Th=0.1)} \\
                       &  & BD-rate            & TS            & BD-rate              & TS              & BD-rate            & TS            & BD-rate               & TS   \\
\hline 
\parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{A \scriptsize{(3840$\times$2160)} }}} 	& {\footnotesize Tango2} 			& 4.03 			& 38.56 			& 2.70 			& 25.95 			& 2.77 			& 37.08 			& 1.82 			& 26.77 \\
																								& {\footnotesize FoodMarket4} 		& 1.74 			& 46.12 			& NA 			& NA 				& 1.71 			& 40.50 			& 1.09 			& 29.40 \\
																								& {\footnotesize Campfire} 			& 3.17 			& 38.23 			& 0.58 			& 7.36 				& 0.73 			& 23.83 			& 0.56 			& 18.01 \\
																								& {\footnotesize CatRobot1} 		& 6.45 			& 36.84 			& 2.58 			& 25.68 			& 2.76 			& 37.02 			& 2.16 			& 27.89 \\
																								& {\footnotesize DaylightRoad2} 	& 5.63 			& 35.47 			& NA			& NA 				& 2.94 			& 35.21 			& 2.13 			& 25.53 \\
																								& {\footnotesize ParkRunning3} 		& 2.10 			& 26.45 			& NA			& NA 				& 1.27 			& 35.25 			& 0.89 			& 29.30 \\
\cline{2-10}	                                                                                                                                                                                            
																										   & {\textbf{Average}} 	& \textbf{3.85} & \textbf{36.46} 	& \textbf{1.95} & \textbf{16.99} 	& \textbf{2.03} & \textbf{34.36} 	& \textbf{1.44} & \textbf{25.81} \\
\hline 	                                                                                                                                                                                                    
	                                                                                                                                                                                                        
\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{B \scriptsize{(1920$\times$1080)} }}} 	& {\footnotesize MarketPlace} 		& 4.33 			& 33.64 			& 1.33 			& 23.25 			& 2.36 			& 45.05 			& 1.60 			& 37.03 \\
																								& {\footnotesize RitualDance} 		& 3.55 			& 34.17 			& 0.92 			& 16.35 			& 1.65 			& 46.60 			& 1.17 			& 39.28 \\
																								& {\footnotesize Cactus} 			& 5.72 			& 29.36 			& 0.82 			& 13.80 			& 1.25 			& 39.28 			& 0.90 			& 34.88 \\
																								& {\footnotesize BasketballDrive} 	& 3.30 			& 37.28 			& 0.99 			& 15.65 			& 1.75 			& 39.31 			& 1.17 			& 33.24 \\
																								& {\footnotesize BQTerrace} 		& 1.90 			& 20.21 			& 0.67 			& 13.54 			& 0.49 			& 30.79 			& 0.39 			& 19.27 \\
\cline{2-10}                                                                                                                                                                                                
																								& \textbf{Average} 					& \textbf{3.76} & \textbf{30.27} 	& \textbf{0.95} & \textbf{16.19} 	& \textbf{1.50} & \textbf{39.80} 	& \textbf{1.05} & \textbf{31.80} \\
\hline                                                                                                                                                                                                      
\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{C \scriptsize{(832$\times$480)} }}} 	& {\footnotesize BasketballDrill} 	& 2.29 			& 29.23 			& 0.19 			& 7.43 				& 0.47 			& 33.93 			& 0.37 			& 23.71 \\
																								& {\footnotesize BQMall} 			& 2.69 			& 27.48 			& 0.12 			& 3.99 				& 0.44 			& 36.75 			& 0.41 			& 24.07 \\
																								& {\footnotesize PartyScene} 		& 2.22 			& 20.80 			& -0.10 		& 2.88 				& 0.17 			& 22.75 			& 0.13 			& 15.77 \\
																								& {\footnotesize RaceHorses} 		& 3.02 			& 26.39 			& 0.15 			& 3.16 				& 0.76 			& 30.27 			& 0.49 			& 22.84 \\
\cline{2-10}                                                                                                                                                                                                
																								& \textbf{Average} 					& \textbf{2.56} & \textbf{25.77} 	& \textbf{0.09} & \textbf{4.05} 	& \textbf{0.46} & \textbf{30.44} 	& \textbf{0.35} & \textbf{21.29} \\
\hline                                                                                                                                                                                                      
\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{D \scriptsize{(416$\times$240)} }}} 	& {\footnotesize BasketballPass} 	& 1.85 			& 26.97 			& 0.06 			& 3.37 				& 0.32 			& 28.29 			& 0.25 			& 15.37 \\
																								& {\footnotesize BQSquare} 			& 1.61 			& 14.86 			& 0.09 			& 3.54 				& 0.34 			& 20.54 			& 0.25 			& 5.70 \\
																								& {\footnotesize BlowingBubbles} 	& 3.03 			& 22.15 			& 0.12 			& 3.59 				& 0.37 			& 26.31 			& 0.20 			& 14.69 \\
																								& {\footnotesize RaceHorses} 		& 2.92 			& 24.20 			& 0.16 			& 0.70 				& 0.39 			& 33.73 			& 0.23 			& 14.37 \\
\cline{2-10}                                                                                                                                                                                                
																								& \textbf{Average} 					& \textbf{2.35} & \textbf{21.53} 	& \textbf{0.11} & \textbf{2.34} 	& \textbf{0.36} & \textbf{26.80} 	& \textbf{0.23} & \textbf{11.66} \\
\hline                                                                                                                                                                                                      
 \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{E \scriptsize{(1280$\times$720)} }}}  	& {\footnotesize FourPeople} 		& 2.31 			& 33.77 			& NA			& NA				& 0.88 			& 42.94 			& 0.71 			& 20.60 \\
																								& {\footnotesize Johnny} 			& 3.53 			& 35.22 			& NA			& NA				& 1.56 			& 39.83 			& 1.01 			& 19.45 \\
																								& {\footnotesize KristenAndSara} 	& 2.58 			& 36.50 			& NA			& NA				& 1.25 			& 42.05 			& 0.86 			& 25.44 \\
\cline{2-10}                                                                                                                                                                                                
																								& \textbf{Average} 					& \textbf{2.81} & \textbf{35.15} 	& \textbf{NA}	& \textbf{NA}		& \textbf{1.23} & \textbf{41.59} 	& \textbf{0.86} & \textbf{21.68} \\
\hline                                                                                                                                                                                                      
																						\multicolumn{2}{c|}{\textbf{Total average}} & \textbf{3.18} & \textbf{30.63} 	& \textbf{0.71} & \textbf{7.12} 	& \textbf{1.21} & \textbf{35.27} 	& \textbf{0.85} & \textbf{24.18} \\
 \hline
 \hline
\end{tabular}
\label{tab:result}
\end{table*}

